Answering Ambiguous Questions through Generative Evidence Fusion and Round-Trip Prediction

In open-domain question answering, questions are highly likely to be ambiguous because users may not know the scope of relevant topics when formulating them. Therefore, a system needs to find possible interpretations of the question, and predict one or multiple plausible answers. When multiple plausible answers are found, the system should rewrite the question for each answer to resolve the ambiguity. In this paper, we present a model that aggregates and combines evidence from multiple passages to adaptively predict a single answer or a set of question-answer pairs for ambiguous questions. In addition, we propose a novel round-trip prediction approach to iteratively generate additional interpretations that our model fails to find in the first pass, and then verify and filter out the incorrect question-answer pairs to arrive at the final disambiguated output. Our model, named Refuel, achieves a new state-of-the-art performance on the AmbigQA dataset, and shows competitive performance on NQ-Open and TriviaQA. The proposed round-trip prediction is a model-agnostic general approach for answering ambiguous open-domain questions, which improves our Refuel as well as several baseline models. We release source code for our models and experiments at https://github.com/amzn/refuel-open-domain-qa.

==> fig/fig_model_old.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{1.0\linewidth}
\includegraphics[width=\linewidth]{fig/pipeline.pdf}
\caption{Overall Pipeline of \modelnameshort. The Answer Prediction module and Question Disambiguation module are detailed in (b) and (c).}\label{fig:pipeline}
\end{subfigure}
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{fig/ap.pdf}
\caption{Answer Prediction Module}\label{fig:ap}
\end{subfigure}
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{fig/qd.pdf}
\caption{Question Disambiguation Module}\label{fig:qd}
\end{subfigure}
\caption{The overall diagram of our proposed \modelnameshort. 
% and the architecture of its Answer Prediction Module and Question Disambiguation Module.
% Given the prompt question $Q^p$, \modelnameshort\ first retrieves and reranks N question-relevant passages (Section \ref{sec:rrrk}). Then, taking the top K passages and prompt question $Q^p$, the answer prediction module \ref{fig:ap} generates one or multiple answers (Section \ref{sec:ap}). If more than one answer is predicted, the question disambiguation module \ref{fig:qd} generates a disambiguated question $Q^d_i$ for each predicted answer $A_i$ (Section \ref{sec:qd}).
}
% \vspace{-0.1in}
\label{fig:model}
\end{figure*}

==> fig/fig_roundtrip_old.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{fig/roundtrip.pdf}
\caption{The process for round-trip generation. Generated disambiguated questions $Q^d$ are further taken as the input of our pipeline to find more interpretations. If the generated question $Q^d$ still has multiple interpretations, the newly predicted answers will receive their own questions. (AP, QD are the Answer Prediction module and Question Disambiguation module of \modelnameshort, respectively)}
\label{fig:roundtrip}
% \vspace{-0.1in}
\end{figure*}

==> tab/tab_ablation_ap.tex <==
\begin{table}[!t]
    \small
    \centering
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l c c c }
    \toprule
    Models & \# QAs & \Fanswer\ (all) & \Fanswer\ (multi) \\
    \midrule
    \modelnameshort\    & 1.55 & \textbf{48.4} & \textbf{37.0}   \\
    ~~~w/o \ambignq\  & 1.00 & 44.3 & 29.4     \\
    ~~~only \ambignq\   & 1.60 & 45.0 & 34.4  \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    Ablation Study of the answer prediction module on the dev. set. ``w/o \ambignq'' is the model pre-trained on the \nqopen\ dataset without fine-tuned on \ambignq, ``only \ambignq'' is the model only trained on \ambignq.
    }
    % \vspace{-0.1in}
    \label{tab:ablation_aq}
\end{table}

==> tab/tab_diff_psgs.tex <==
\begin{table}[!t]
    \small
    \centering
    \resizebox{0.9\columnwidth}{!}{
    \begin{tabular}{c | c c c  c c }
    \toprule
    \#Psgs & \#QAs & \Fanswer\ (all) & \Fedit\ & Comb. \\
    \midrule
    10    & 1.39 & 46.8 & 10.3 & 57.1       \\
    25    & 1.56 & 47.6 & 10.9 & 58.5     \\
    50    & 1.50 & 48.2 & 11.1 & 59.3     \\
    100   & 1.55 & \textbf{48.4} & \textbf{11.2} & \textbf{59.6}    \\
    \bottomrule
    \end{tabular}
    }
    \caption{
    Performance of \modelnameshort\ on the development set as a function of the number of input passages (\#Psgs). ``\#QAs'' denotes the average number of generated QA pairs per prompt question.
    }
    \label{tab:diff_psgs}
    % \vspace{-0.2in}
\end{table}
